Statistically Efficient Variance Reduction with Double Policy Estimation for Off-Policy Evaluation in Sequence-Modeled Reinforcement Learning

Offline reinforcement learning aims to utilize datasets of previously gathered environment-action interaction records to learn a policy without access to the real environment. Recent work has shown that offline reinforcement learning can be formulated as a sequence modeling problem and solved via supervised learning with approaches such as decision transformer. While these sequence-based methods achieve competitive results over return-to-go methods, especially on tasks that require longer episodes or with scarce rewards, importance sampling is not considered to correct the policy bias when dealing with off-policy data, mainly due to the absence of behavior policy and the use of deterministic evaluation policies. To this end, we propose DPE: an RL algorithm that blends offline sequence modeling and offline reinforcement learning with Double Policy Estimation (DPE) in a unified framework with statistically proven properties on variance reduction. We validate our method in multiple tasks of OpenAI Gym with D4RL benchmarks. Our method brings a performance improvements on selected methods which outperforms SOTA baselines in several tasks, demonstrating the advantages of enabling double policy estimation for sequence-modeled reinforcement learning.

==> 0Algo.tex <==
\begin{algorithm}[h]
    \caption{pseudocode for DPE}
    \begin{algorithmic}[1]
        \State {Initiate behavior policy estimator $\hat{\pi}_{b}$}
        % \For{$k = 0 $ to $pretrain\_steps$}                    
        \While {$\hat{\pi}_{b}$ not converged}

        \EndWhile
        \State {Random Sample Trajectories: $ H \sim \mathrm{D}$}
        \State {Estimate the behavior policy in $\mathcal{D}$ as $\hat{\pi_b} := \text{argmax} \sum_{H \in \mathcal{D}} \sum_{t=0}^{L-1} \text{log}\pi(a| H_{t-n:t})$.}
            % \State {Sample time index for each trajectory: $h \sim [1,L]$}
            % \State {Calculate Loss: $\mathcal{L}(\hat{\theta}) = \sum_{s_t, a_t, h} \pi_{\theta}(a_t|s_t)$} 
            % \State {Update behaviour policy estimator  parameters: $\theta = \theta + \eta \nabla_{\theta}(\mathcal{L}(\theta))$}
        % \EndFor   
        \State {initialize Decision Transformer $\pi_{DT}$ and its estimator $\hat{\pi_t}$}
        \For{$k = 0 $ to $max\_train\_steps$}
            \State {Random Sample Trajectories: $\tau \sim \mathrm{D}$}
            \State {Sample time index for each trajectory: $h \sim [1,L]$}
            \State {Generate Trajectories from DT: $\hat{a} =\pi_{DT}(s_{-K,k},r_{-K,k}))^2$}
            % \State {Calculate weighted Loss for DT: $\mathcal{L}(\Tilde{\theta}) = \frac{\hat{\pi}_t(a_i,s_i)}{\hat{\pi}_b(a_i,s_i)}\frac{1}{N}\sum_{i=1}^{N}(\hat{a_i}-a_i)^2$}
            % \State {Sample Trajectories from DT:}
            \State {Estimate $\nabla_{\theta} J(\pi_{DT}) = \frac{1}{K}\sum_{k} \frac{\hat{\pi}_t(a_k,s_k)}{\hat{\pi}_b(\hat{a_k},s_k)}\nabla_{\theta_{DT}} (a_k - \hat{a})^2$}
            \State {Update Decision Transformer: $\theta_{\pi_{DT}} = \theta_{\pi_t}  + \eta \nabla_{\theta_t}J(\pi_{\theta_t})$ }
            \State {Update Target policy Estimator: $\theta_{\hat{\pi}_t }= \eta \nabla_{\hat{\theta}_t}J(\pi_{\hat{\theta}_t})$ }
        \EndFor
        \State {Return Decision Transformer $\pi_t$}
    \end{algorithmic}
\end{algorithm}


